Resolution Complete In-Place Object Retrieval given Known Object Models

This work proposes a robot task planning framework for retrieving a target object in a confined workspace among multiple stacked objects that obstruct the target. The robot can use prehensile picking and in-workspace placing actions. The method assumes access to 3D models for the visible objects in the scene. The key contribution is in achieving desirable properties, i.e., to provide (a) safety, by avoiding collisions with sensed obstacles, objects, and occluded regions, and (b) resolution completeness (RC) - or probabilistic completeness (PC) depending on implementation - which indicates a solution will be eventually found (if it exists) as the resolution of algorithmic parameters increases. A heuristic variant of the basic RC algorithm is also proposed to solve the task more efficiently while retaining the desirable properties. Simulation results compare using random picking and placing operations against the basic RC algorithm that reasons about object dependency as well as its heuristic variant. The success rate is higher for the RC approaches given the same amount of time. The heuristic variant is able to solve the problem even more efficiently than the basic approach. The integration of the RC algorithm with perception, where an RGB-D sensor detects the objects as they are being moved, enables real robot demonstrations of safely retrieving target objects from a cluttered shelf.

==> draft0.tex <==
{\bf Objective:} The goal of this project is to study 
%which modes of human-robot communication are most effective for task specification and 
how to best utilize task specification strategies in a task and motion planner. Specifically, the focus will be on combining voice and gesture communication to simply describe a rearrangement/assembly task. Additionally, since many tasks will initially be under-specified, it will be necessary to include two-way communication so that the robot can query for missing details in the task (e.g. final orientation of objects). Thus, task planning will involve balancing verbal query and object manipulation so as to discover and execute a task.

%\kostas{I think the first question is great but it is probably too large of a scope for one person and you will need to work with others on this aspect. My suggestion is to focus on the 2nd question. Lets pick a setup of task specification that we believe is natural for a non-expert and deal with how task and motion planning can effective achieve this specification given ambiguity and dynamic changes in the specification. Notice that I changed the title.}

%\kostas{So, key question here that needs to be answered in your following paragraph: How does the non-expert specify a task?}

{\bf Task Environment:} The task environment will feature one human agent and one robot agent (with multiple arms) surrounding a table. Within this environment the mobility and reachability of the robot can be varied. For simplicity of modeling physical human-robot interaction, it will be assumed that the robot and human are restricted to opposite sides of the table but that both can reach across the table to touch objects placed in front of one or the other. This environment allows for easy verbal and gesture based interaction while including a basic safety barrier (the table) to minimize human-robot collision.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/task_environment.png}
    \caption{A simulated scene of the task environment. In this example, Baxter observes a human pointing at a cup.}
    \label{fig:task_environment}
\end{figure}

%\kostas{I like the setup of 1 person, 1 dual-arm robot and a tabletop, where the person and the robot are on opposite sides. It is rather and clear straightforward. It allows for interaction but it also introduces a safety barrier. You may want to introduce some of this justification in the text above.}

%\kostas{What robot in the lab do you want to use for this task? This will affect whether we are talking about a mobile manipulator or a static one. Lets make the setup concrete given our lab resources, e.g., Baxter at the front desk or Motoman inside the lab in front of a table. This will help to clarify what is the next step here and you can expand upon this document with an actual image of the setup. }

{\bf Challenges:}
Besides the classic challenges of rearrangement planning, the introduction of human interaction introduces both task and motion planning challenges. In terms of motion planning, the robot must not collide with the human; this requires online collision checking and replanning. In fact, replanning the motion is not the only possible resolution to an imminent collision with the human; alternatively the robot can halt and communicate to the human that they are in the way and resume motion once they move away. This example begins to highlight the task planning challenges introduces by the human agent. Normally task planning only needs to answer ``when do I do?'' and ``when do I sense?'', but with the human involved, task planning needs to additionally answer ``what do I do?'', ``what do I say?'', ``when do I say and when do I do?''.

In addition to planning challenges, there are challenges of basic natural language processing/generation and perception/interpretation of human actions (pointing, touching, grasping).

\kostas{Lets not emphasize first tasks where the robot and the human are solving them together, where collision avoidance of the human motion is important. We can get into that incrementally.}

\kostas{Lets focus first on setups where the person is just specifying a task (e.g., through pointing, talking, etc.). The need for replanning may still arise but not because of safety considerations and collisions between the robot and the person. It will arise because of ambiguous specification of the task and the need for the robot to understand better the true objective of the person.}

\kostas{You should also be thinking of a very specific problem, such as setting up a dinner table. What are the objects involved? What will the person have to specify? What will the robot have to infer from the specification?}

\kostas{Not sure whether we should consider dialog from scratch or not. Should the robot ask every time that there is ambiguity for clarification? Or should our first attempt be: execute something given the best inference from what it has been specified and then the person can intervene and correct what is happening?}

\kostas{You cannot solve all of the problems related to this problem, i.e., planning + perception + language processing. Initially, you should try to solve the problem in simulation, where the language will be text provided by a human in a very limited vocabulary. If you want to introduce pointing, the user should be able to click in the simulation environment in order to point. When we move to the real setup, you can replace these components. Bowen or someone else may be able to help with understanding pointing. And we will need Matthew or someone else to contribute on the NLP side of things. Your focus should be on the decision making side of things.}

{\bf Related Work:} Recently pre-determined human-robot collaborative tasks has been tackled by answer-set programming paradigms mixed with hierarchical planning techniques \cite{rizwan2020human, faroni2020layered}. Such approaches require ``atoms'' that are somewhat specialized for the predefined task. Focusing more on the communication side, \cite{unhelkar2020decision} and similar works use a partially observable Markov decision process (POMDP) to model human-robot interaction. The POMDP in such approaches factor the action space and transition function into movement actions and communication actions (usually verbal). Such models also require task specific defined states/actions in order to be computationally tractable.
In \cite{raessa2020human}, a human robot assembly system is proposed that efficiently distributes sub-tasks between the human and robot; the capabilities of each are known before hand. 

\kostas{Thanks for the references. I took a quick look in them.}

\kostas{Volkan and Esra sure like "answer set programming"... it is their favorite tool! Their overall setup is interesting as it includes sensing and communication actions. The tree of conditional actions is a useful representation of the problem. We can adopt the hybrid conditional planning framework but perhaps allow ourselves to pick alternative methods for planning.}

\kostas{The two layer approach of Faroni et al. is reasonable. The focus here is more on the replanning aspects and the execution in the context of a collaborative task. Given what I mentioned above, I would like us to first see the case where the human specifies the task and the robot executes it. Some of the ideas here are still useful and the mosaic challenge is interesting. }

\kostas{Julie Sha's group is definitely one we should be paying attention to in this line of work. For sure, all of these problems can be modeled as POMDPs. But given the computational complexity of such problems, the critical issue is indeed how to factor the space so as to bring down the complexity. The focus in ref. 3 seems to be on the bidirectional communication, which again I am not sure whether this should be our starting point.}

\kostas{Kensuke Harada also has a long history in manipulation and assembly tasks. His group tends to use tools that are much closer to the ones we have been using, e.g., sampling-based planning for the low level motion planning and then some form of search or automaton for the high-level planning. The focus here is on how to distribute the tasks between the robot and the human for a collaborative problem. See what you can learn from this work in terms of a task that is executed by the robot given an ambiguous human specification.}

In \cite{wang2019symbiotic}, a taxonomy of human robot collaboration (HRC) is described and future research directions suggested. The directions that this work will focus on primarily is programming-free robot control. It is noted in \cite{wang2019symbiotic} that using gesture and voice commands alone are not practical for successful HRC especially in a noisy work environment. Rather it could be fruitful to combine learned human behavior intent models with a variety of event triggers such as voice, gaze, gestures, brain-waves, and haptic control.

\kostas{Thanks as well for the survey. I encourage you to share it with others in the emailing list and give some context of why you looked into it. For the "dinner table setup problem" as ambiguously specified by a human, are we in the "interaction" or "cooperation" area?  It was interesting to read the point from this survey that you brought up (i.e., gesture+voice not being good in noisy environments). I think we can also skip such considerations as noisy environments for now. Was this in the context of a collaborative task? The following sentence in your document talking about "learned human behavior intent models" made me believe so.}

\kostas{Make sure that you keep track of an active bibliography in this domain - this will be very useful for any paper submission as well as a quick reference as we may want to consider how to approach different challenges in this domain. The best way forward is to identify one state-of-the-art paper that we believe deals with the setup closest to the one we want to address. Then, see what are the gaps in that solution that we can improve upon. As you do an additional round of literature search, think of this objective and let me know 1-3 directions that we could consider.}

{\bf Misc. Ideas:}

Experiments/Tasks in consideration
\begin{itemize}
    \item Mosaic/Puzzle: similar to \cite{faroni2020layered} but with the user showing a picture of complete puzzle to the robot camera. Human can correct misplaced pieces or verbally communicate mistakes. Robot needs to communicate confidence of piece placement and ask for help when not confident.
    
    \item Setting a table: Human can specify one persons plate/utensils with picture or by demonstration. Robot replicates for N people. Human can communicate when robot messed up or directly fix a robots mistake and the robot would need to react to these passive or active directives.
    
\end{itemize}

\kostas{I tend to prefer the "setting a table" because it gets closer to a real application. But I am not sure about the specification of the problem via a picture or via demonstration for now. }

Methods of Communication to consider:
\begin{itemize}
    \item Verbal
    \item Gesture
    \item Haptic
    \item Gaze (to what precision?)
    \item Photographs
    \item Facial expressions?
\end{itemize}

\kostas{Let me know what you think about the following given what you have read and what you would like to do. I am thinking of this in a simulation environment first. As input we can have: a) a set of objects and their current locations, b) a semantic label for each object (e.g., "plate", "fork", etc.) - note that we can have multiple instances of the same object category - c) a text description provided by a non-expert that specifies how to setup a table with these objects and a limited vocabulary of words (such as "pick", "place", "left/right", etc.) d) optionally: the user can also point by clicking on specific objects and associate words in the text description with clicks. You could first try to setup a planning and execution framework that does its best with the specification. Then, we can look into additional communication by the user during or after the execution of the plan by the robot, where through additional verbal/text descriptions and pointing actions, the person is trying to correct the placement of objects.}

How to extend previous approaches?:

\kostas{This is key. We should find the most relevant work and build on top of that.}

I think extending the grammar based approaches to reason about goal states differently could work. Keeping some model of current human satisfaction could be used to guide the robot to plan to make actions that progress towards the goal. The general question is how to model when the robot should be learning what the goal is and when it should be acting to achieve it. Based on \cite{wang2019symbiotic} it seems that the approach to try is to have pre-programmed triggers (in the form of verbal,gesture,etc.) to tell the robot to stop and then collect an aggregate of data during this observation mode to feed into a more complex model designed to determine the goal. What I still don't know is what this goal determining model should be; could I come up with a metric on the human-robot state space or perhaps a reinforcement learning model with a reward for successful completion (e.g. thumbs up from the human). Or, should I start with more explicit models: initialize goal belief from a photograph and then refine based on human communicated corrections.

\kostas{These sounded like important questions but I am not sure I followed everything here. Perhaps iterate given the above feedback and we discuss about these questions online.}

==> draft1.tex <==
{\bf Introduction}

Robots have widely been used in factories and warehouses to carry out repetitive tasks with high precision. As robot hardware becomes cheaper it will become possible for people to afford robots that help automate chores at home. In order for such robots to be useful for multiple tasks, people without programming and robotic experience will need a way to instruct robots to perform everyday tasks through a natural interface. In this work, a task specification method is proposed that is able to ground natural language to the domain of pick and place tasks.

{\bf Related Work}

Initial approaches to task specification involved translating natural language directly into logical statements about system state \cite{raman2013sorry}. These approaches were effective at determining viability of tasks and explaining when and how a given task specification was infeasible. Such approaches, however, did not handle possible ambiguity in the user defined specifications. Thus, the next set of approaches developed multiple probabilistic models to account for task ambiguity by maximizing likelihoods \cite{paul2018efficient} or minimizing ``energy'' \cite{misra2016tell}. Recently, data driven learning approaches have been proposed for various interactive pick and place tasks \cite{hatori2018interactively,shridhar2018interactive,mees2021composing}. These approaches deal with ambiguity by requesting clarification when the task is under-specified. While the learned approaches are better suited at dealing with ambiguity of task specification, they abandon explicit reasoning over task feasibility. Is there a method that can handle both task ambiguity and feasibility?

{\bf Method}

The proposed method will take as input text in natural language and parse it into dependency trees \footnote{\url{https://en.wikipedia.org/wiki/Dependency_grammar}}.
Next object relations will be extracted into a graph with nodes as objects and directed edges describing geometric relations (possibly ambiguous) between the source object and target object. Note, this can be done dynamically, by inserting edges phrase by phrase. Figure~\ref{fig:relation_graph} shows an example of the extracted graph structure for a table setting task. 

To deal with ambiguity of object positions with relation to one another, a set of constraints is enforced based on the following principles.
\begin{enumerate}
    \item Feasibility - objects remain on the table (consider stability for more complicated scenarios)
    \item Symmetry - An object between two other objects should be equally spaced between them unless otherwise specified. This can be applied recursively. For example if I ask the box A is to be put between box B and C but closer to B, then this symmetry would collapse the ambiguity of the position of box A to half way between the half way point between B and C.
    \item Repulsion - unless constrained by above or objects are supposed to touch, enforce a buffer around an object of a quarter of its ``effective diameter''.
    \item Attraction - after all other constraints are satisfied, prefer objects that share a direct positional relation to be as close to one another as possible.
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/graph.png}
    \caption{An example geometric relation graph for a table setting task. In this example, the plate is the object of reference.}
    \label{fig:relation_graph}
\end{figure}

In addition to ambiguity in geometric relations between objects there may also be ambiguity of intrinsic object orientation. To address these types of ambiguity we enforce the principle of axis alignment...  

{\bf Task Environment}

The task environment will feature one human agent and one robot agent (with multiple arms) surrounding a table. Within this environment the mobility and reachability of the robot can be varied. For simplicity of modeling physical human-robot interaction, it will be assumed that the robot and human are restricted to opposite sides of the table but that both can reach across the table to touch objects placed in front of one or the other. This environment allows for easy verbal and gesture based interaction while including a basic safety barrier (the table) to minimize human-robot collision.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/task_environment.png}
    \caption{A simulated scene of the task environment. In this example, Baxter observes a human pointing at a cup.}
    \label{fig:task_environment}
\end{figure}


{\bf Evaluation}
First, multiple goal scenes consisting of basic objects such as blocks, puzzle pieces, and tableware, will be generated both manually and randomly. For each unique scene, a human will be tasked to write instructions for another human to produce the given scene starting from an empty table. These instruction will then be given to the robot and the final poses of each object in the manipulated scene and the goal scene will be compared. Furthermore, the same instructions will be given to different human than the one who wrote the instruction and the persons final scene will also be compared to that of the robot's and to the original goal.

==> draft2.tex <==
%{\bf Motivation}
%Robots have widely been used in factories and warehouses to carry out repetitive tasks with high precision. As robot hardware becomes cheaper it will become possible for people to afford robots that help automate chores at home. In order for such robots to be useful for multiple tasks, people without programming and robotic experience will need a way to instruct robots to perform everyday tasks through a natural interface. In this work, a task specification method is proposed that is able to ground natural language to the domain of pick and place tasks.



{\bf Problem Statement}

The state of a rigid 3D object is describable as a point (or configuration) in $SE(3)$, which is a 6D space expressing both the translation and rotation of the object. For an environment with $n$ objects with configurations $s_0,s_1,...,s_n \in SE(3)$ the problem of object rearrangement involves finding a sequence of motions $\pi_0,\pi_1,...,\pi_m : [0,1] \to \Cspace$ for a robot arm to move the objects from their starting configurations to some given goal configurations $g_0,g_1,...,g_n \in SE(3)$. More generally, we can consider a collection of valid goal configurations per object $G_0,...,G_n \subset SE(3)$. This work, however, considers the case where such sets of goal configurations are not explicitly given but are rather implicitly described through natural language. Thus, before solving the task and motion planning problem of rearranging objects we need to translate a natural language description into a set of valid goal configurations per object.

As a first step in this direction and in order to focus on the task of natural language grounding, this work first considers the simpler task of reorienting objects on a tabletop. In this setting, the translation of the objects is the same in both the start and goal configurations. Furthermore, the objects are far enough apart so that they will not collide for any orientation. Instead of full poses in $SE(3)$ the focus is on transforming the initial object orientations $d_0,...d_n \in SO(3)$ into the respective goal orientation set $H_0,...,H_n \subset SO(3)$. The motion planning challenge of grasping and placing an object is simplified in this task environment as each object has sufficient collision free space around it. The challenge of interpreting and grounding the language instructions describing object rotations is still interesting and has not been explicitly studied to the best of our knowledge.

{\bf Outline of Online Steps to Tackle this Problem}
\begin{enumerate}
    \item Generate a set of stable orientations $st_0, \ldots, st_n \subset SO(3)$ for each object given the supporting surface.
    \item Given a natural language instruction: 
    \begin{itemize}
        \item Identify first the object $o_i$ that the instruction refers to (we will provide a vocabulary to human instructors on how to refer to objects, e.g., "blue cylinder" or the "black cube"). 
        \item Then, the core challenge is to map the natural language instruction to a valid subset $v_i \subset SO(3)$. There are multiple methods to consider here on how to learn this mapping offline - see section below on Related Work.
    \end{itemize}
    \item Rank stable object poses $st_i$ by distance to the valid subsets $v_i$ of $SO(3)$ according to the instruction.
    \item Prune poses in $st_i$ with a  distance greater than some threshold $\delta$ from the valid subsets $v_i$.
    \item Iterate through the remaining poses in $st_i$ according to their ranking and generate motion plans to reorient them. 
    \item Execute the first successful motion plan.
\end{enumerate}

{\bf Related Work on Grounding Language Instructions}
Initial approaches to grounding natural language robot task descriptions approached the problem as a translation problem. They would use sentence parsers to transform sentences in natural language into a more formal language, such as LTL \cite{raman2013sorry} or semspec \cite{pomarlan2018robot}, and then apply cleverly constructed grammars to parse the intermediate languages into an executable program for a given robot system. Such approaches have the benefit of handling multiple failure modes in task specification and can be used to produce explanations of why a given task was found to be invalid. Drawbacks of such approaches are their complexity in adapting to new robot systems and ability to handle ambiguity in user descriptions.

In order to address ambiguity in language input some approached the problem of grounding natural language descriptions through Bayesian inference by constructing factor graphs from a given sentence parsing. Such approaches inferred either robot actions directly \cite{tellex2011understanding}, constraints on the workspace \cite{howard2014natural, paul2018efficient}, which were passed to a conventional motion planner, or formal clauses \cite{misra2016tell} which are evaluated into an executable plan. These techniques are more adaptable to a larger variety of language input but have trouble scaling with workspace complexity.% due to an explosion of factors.

More recently data driven approaches have tackled natural language grounding. Some use demonstrations to learn reward functions for Object Oriented Markov Decision Problems (OO-MDPs) via inverse reinforcement learning (IRL) \cite{macglashan2015grounding, arumugam2017accurately, arumugam2019grounding}. Others have also proposed end-to-end deep neural networks that directly learn and tie together perception and language models \cite{shridhar2018interactive, hatori2018interactively, mees2021composing}.

{\bf Experimental Setup}
First, multiple goal scene categories consisting of objects with basic shapes, such as blocks and cylinders, will be generated where the objects are assigned locations on a tabletop. For each scene category, a set of instances will be generated by scrambling the orientations of the objects but guaranteeing that the objects are lying stable on the tabletop. From each scene category, a start and a goal scene instance will be randomly selected and presented to a human. The human will be asked to write instructions for a robot to manipulate the objects so as to take them from the start scene configuration to the goal configuration. These instructions will then be presented to the robot for the above steps to be executed. The final poses of each object in the manipulated scene and the goal scene will be compared via inverse cosine distance. 
%( or something else \cite{huynh2009metrics}?)

Such an experiment setup may be flawed, however, as humans might consider multiple goal scenes with similar features to be considered equivalent in value and thus give similar or equivalent instructions for such scenes. Thus, in addition to measuring distance between the given goal scene and the produced goal scene, we can also survey participants on how successful the robot executed their instructions. In addition, we could query participants to reorient the objects in the scene to produce multiple configurations that they consider satisfactory, and then take the average $SO(3)$ distance between the robot-produced scene and the human-produced scenes.

==> draft3.tex <==
%{\bf Motivation}
%Robots have widely been used in factories and warehouses to carry out repetitive tasks with high precision. As robot hardware becomes cheaper it will become possible for people to afford robots that help automate chores at home. In order for such robots to be useful for multiple tasks, people without programming and robotic experience will need a way to instruct robots to perform everyday tasks through a natural interface. In this work, a task specification method is proposed that is able to ground natural language to the domain of object retrieval.


{\bf Problem Statement}
The state of a rigid 3D object is describable as a point (or configuration) in $SE(3)$, which is a 6D space expressing both the translation and rotation of the object. For an environment with $n$ objects with configurations $s_0,s_1,...,s_n \in SE(3)$ the problem of object rearrangement involves finding a sequence of motions $\pi_0,\pi_1,...,\pi_m : [0,1] \to \Cspace$ for a robot arm to move the objects from their starting configurations to some given goal configurations $g_0,g_1,...,g_n \in SE(3)$. More generally, we can consider a collection of valid goal configurations per object $G_0,...,G_n \subset SE(3)$.

For the specific task of object retrieval, some of the object start configurations may be unknown due to object occlusions. Furthermore, the goal configurations aren't final as the task of object retrieval may require multiple arrangement before the target object is discovered. In order to bypass a brute force search for object discovery, this work proposes using information from natural language descriptions of target objects to influence the planning process. For example, if a human requests, ``pick up the green apple behind the cereal box'', then the planner should be able to deduce to move the cereal box out of the way in order to find the target object (green apple).

In addition to using information only from the original instruction, the planner integrates a full conversational agent to occasionally query the user for more information. More queries could be useful when either a human gives contradictory (or seemingly contradictory) information, the initial human description was vague, or the object discovery is taking too long (too many wrong guesses).

Assumptions:
 - 

TODO: define dependency graph + add figure

{\bf Outline of Online Steps to Tackle this Problem}
\begin{enumerate}
    \item Query the user for a target object.
    \item Parse the user's description and deduce any hints to the objects location in the scene.
    \item \label{item:loop} Given current sensing of the environment + the parsing of user hint (if any). Construct a dependency graph where each node represents an object and each directed edge represents a relation that necessitates moving the target object before the source object.
    \item Perform a DFS from the target object node (or another source node if no hint was provided) to retrieve an ordering of object manipulations.
    \item For each object in the ordering, pick it up, re-sense, and place it somewhere that minimizes further object occlusion (TODO). 
    \item Repeat from step \ref{item:loop} until object is visible. (optionally query the user for additional information at various iterations depending on preference of saving human time vs robot time)
\end{enumerate}

%{\bf Related Work on Grounding Language Instructions}
%Initial approaches to grounding natural language robot task descriptions approached the problem as a translation problem. They would use sentence parsers to transform sentences in natural language into a more formal language, such as LTL \cite{raman2013sorry} or semspec \cite{pomarlan2018robot}, and then apply cleverly constructed grammars to parse the intermediate languages into an executable program for a given robot system. Such approaches have the benefit of handling multiple failure modes in task specification and can be used to produce explanations of why a given task was found to be invalid. Drawbacks of such approaches are their complexity in adapting to new robot systems and ability to handle ambiguity in user descriptions.

%In order to address ambiguity in language input some approached the problem of grounding natural language descriptions through Bayesian inference by constructing factor graphs from a given sentence parsing. Such approaches inferred either robot actions directly \cite{tellex2011understanding}, constraints on the workspace \cite{howard2014natural, paul2018efficient}, which were passed to a conventional motion planner, or formal clauses \cite{misra2016tell} which are evaluated into an executable plan. These techniques are more adaptable to a larger variety of language input but have trouble scaling with workspace complexity.% due to an explosion of factors.

%More recently data driven approaches have tackled natural language grounding. Some use demonstrations to learn reward functions for Object Oriented Markov Decision Problems (OO-MDPs) via inverse reinforcement learning (IRL) \cite{macglashan2015grounding, arumugam2017accurately, arumugam2019grounding}. Others have also proposed end-to-end deep neural networks that directly learn and tie together perception and language models \cite{shridhar2018interactive, hatori2018interactively, mees2021composing}.

{\bf Related Work}
Object retrieval (sometimes called mechanical search) has had many recent works focus on cluttered and occluded scenes. \cite{bejjani2021occlusion,huang2020mechanical,kurenkov2020visuomotor,danielczuk2019mechanical} that use various models
% TODO: state explicitly which models
to reason over the scene to determine manipulations that will make progress towards the discovery of a target object. This work uses a voxelization of the workspace to reason about object occupancy and occlusion.

Initial approaches integrating natural language descriptions would would use sentence parsers to ``translate'' sentences in natural language into a more formal language, such as LTL \cite{raman2013sorry} or semspec \cite{pomarlan2018robot}, and then apply cleverly constructed grammars to parse the intermediate languages into an executable program for a given robot system. Such approaches have the benefit of handling multiple failure modes in task specification and can be used to produce explanations of why a given task was found to be invalid. Drawbacks of such approaches are their complexity in adapting to new robot systems and ability to handle ambiguity in user descriptions.
The focus of this work is similar in terms of reasoning about feasibility of language instructions but also integrates a conversation agent that could resolve contradictory information or ambiguity.

Other related efforts have used natural language to learn new task primitives \cite{suddrey_teaching_2017} or as input into a hierarchical search process \cite{kurenkov_semantic_2021}. One of the motivations for exploring how a human instruction can complement the partial scene observation is to speed up scene reconstruction and object discovery. To that end, Human-in-the-loop systems \cite{papallas2020non} have been implemented but rely on more direct user interface elements rather than natural language, and don't deal with object occlusion. The proposed work differs by using the language-based task description to inform the planner about the unobserved space.
A recent work \cite{zheng2021spatial} has a similar motivation to integrate language reasoning to speed up task planning for a city-scale navigation environment.
Work on Hierarchical Mechanical Search \cite{kurenkov_semantic_2021} does appear similar to the proposed setup, but handles scene representation and language processing separately, while the current work aims to integrate these two sources of information. 

At least one work does integrate language and task reasoning \cite{nguyen_robot_2020} in order to retrieve objects based on their utility. This work focus not on the object selection but on object discovery within an occluded scene.



{\bf Experimental Setup}
First, multiple objects with basic shapes, such as blocks and cylinders are generated on a tabletop. Some objects are stacked on top of others and a few objects placed purposefully to occlude others. The Baxter robot is put behind the table armed with two parallel grippers big enough to grasp any of the objects on the table. A camera to sense the scene is positioned on the `waist' of the robot with side view of the table (as opposed to from above).

TODO: figure of the scene

==> format/reset_page.tex <==
\newpage
\setcounter{page}{1}
